QT-Opt: Scalable Deep Reinforcement Learning for Vision-Based Robotic Manipulation

In this paper, we study the problem of learning vision-based dynamic manipulation skills using a scalable reinforcement learning approach. We study this problem in the context of grasping, a longstanding challenge in robotic manipulation. In contrast to static learning behaviors that choose a grasp point and then execute the desired grasp, our method enables closed-loop vision-based control, whereby the robot continuously updates its grasp strategy based on the most recent observations to optimize long-horizon grasp success. To that end, we introduce QT-Opt, a scalable self-supervised vision-based reinforcement learning framework that can leverage over 580k real-world grasp attempts to train a deep neural network Q-function with over 1.2M parameters to perform closed-loop, real-world grasping that generalizes to 96% grasp success on unseen objects. Aside from attaining a very high success rate, our method exhibits behaviors that are quite distinct from more standard grasping systems: using only RGB vision-based perception from an over-the-shoulder camera, our method automatically learns regrasping strategies, probes objects to find the most effective grasps, learns to reposition objects and perform other non-prehensile pre-grasp manipulations, and responds dynamically to disturbances and perturbations.

==> arxiv_appendices/ablation_real.tex <==
After prototyping ideas in our simulated setup, we take the best parameters discussed in Appendix~\ref{sec:appendix_ablations_sim}, and repeat those experiments in the real setup, to verify the same parameters carry over across domains. Since real-world finetuning takes considerable robot time, all of these experiments were conducted with entirely off-policy training using a fixed dataset of 580k grasps. The results are therefore in absolute terms worse than the final results of our best policy, but are still useful for understanding the relative tradeoffs of various design choices.

\vspace{-0.1in}
\paragraph{State representation and its effects.}

Echoing results discussed in Appendix~\ref{sec:appendix_ablations_sim} we found that a rich state representation greatly impacts real robot performance. Matching simulated experiments, providing the image, gripper status, and height to bottom of the bin performs better than other representations. These experiments indicate that while hand-eye coordination can in principle be figured out purely from the image observation, explicitly adding domain-specific state features improves performance. We find it very important that such low dimensional state features can be seamlessly integrated into our model, resulting in better performance and data efficiency. All models are trained off-policy for 2.5M steps, with discount $0.9$ and no reward penalty.

\begin{table}[h]
\begin{center}
\begin{tabular}{ |p{12em}|p{7em}| } 
\hline
State Representation & Performance \\
\hline
Image only & 53\% \\ %
\hline
Image + gripper status & 58\% \\ %
\hline
Image + gripper status + height & 70\% \\ %
\hline
\end{tabular}
\end{center}
\caption{Off-policy ablation over state representation.}
\label{table:state-repr-ablation}
\vspace{-0.25in}
\end{table}
\paragraph{Discount and Reward Definition}
To encourage faster grasps, we experimented with decreasing discount and adding a small reward penalty at each timestep. Again, matching sim results, a reward penalty did better than decreasing the discount factor. All models are trained off-policy on the same dataset for 2.5M steps.
\begin{table}[h]
\label{table:learning-ablation}
\begin{center}
\begin{tabular}{|p{12em}|p{7em}|p{7em}|p{7em}|}
\hline
State Representation & Discount Factor & Reward Penalty & Performance  \\
\hline
Image only & 0.9 & 0 & 53\% \\ %
\hline
Image only & 0.7 & 0 & 28\% \\ %
\hline
Image only & 0.9 & -0.05 & 63\% \\ %
\hline
\end{tabular}
\end{center}
\caption{Off-policy ablation over discount and reward.}
\vspace{-0.3in}
\end{table}
\paragraph{Learned Termination}
We compare a task-specific scripted termination condition with a task-agnostic termination action learned by the policy. Details of the scripted termination and learned termination conditions are in the Appendix \ref{appendix:termination}. The learned termination condition performs better in the off-policy case and on-policy case.
 
\begin{table}[h]
\label{table:termination-ablation}
\begin{center}
\begin{tabular}{|p{12em}|p{9em}|p{7em}|}
\hline
Termination Condition & Training Regime & Performance  \\
\hline
Automatic & off-policy & 81\% \\ 
\hline
Learned & off-policy & 87\% \\ 
\hline
Automatic & on-policy finetuning & 95\% \\ 
\hline
Learned & on-policy finetuning & 96\% \\ 
\hline
\end{tabular}
\end{center}
\caption{Off-policy and on-policy ablation of termination condition.}
\vspace{-0.25in}
\end{table}
\paragraph{Quantitative experiments}
\begin{figure}[h]
    \vspace{-0.05in}
    \centering
    \begin{imgrows}
        \imgrow \img{images/bin-unloading}
        \imgrow \img{images/test_two_protocols_side_by_side}
        \imgrow \img{images/octopus}
    \end{imgrows}
    \caption{Illustrations of the bin emptying experiment (a). The (a, right) shows a very small object getting stuck in the corner and requiring a few attempts to get grasped. The test objects for the bin emptying experiment (b, left) and grasping with replacement experiment (b, right). Note that the objects range greatly in size and appearance, and many are exceedingly difficult to grasp due to small size, complex shapes, and varied material properties. Sequence (c) illustrates a grasp on the legs of a toy octopus,
    getting positive visual feedback and resulting in episode termination by the policy. During further ascent, the octopus slips out of the gripper, and the grasp is labeled as a failure. This is not a principled limitation of our method, as we could have terminated an episode at a larger height to get more robust feedback. Robot's observation $I_t$ is shown in (c).}
    \label{fig:bin_unloading}
    \vspace{-0.2in}
\end{figure}
The performance of our algorithm is evaluated empirically in a set of grasping experiments. As discussed in Section~\ref{sec:quantitative} we follow two experimentation protocols. In one set of the experiments we let 7 robots execute 102 grasps each and then average grasp success. See results in column three of Table~\ref{tbl:quantitative_results}. After a successful trial, the object is randomly dropped back into the bin. In a second protocol we place 28 objects into a bin and let the robot perform 30 grasps without object replacement. This time successfully grasped objects are placed into a spare basket. For the bin unloading protocol we report success rates on the first 10 / 20 / 30 grasps to report on increasingly difficult objects remaining in the bin over the unloading process. As the unloading process progresses, large objects tend to be grasped first and small objects are grasped last. The policy is required to localize the small objects and then make a grasp. The ability of our policy to localize small objects in a very sparse scene is learned solely from data, and was not hand tuned.

The test sets, shown in Fig.~\ref{fig:bin_unloading} (b), consist of objects that pose a variety of challenges for grasping. They range in size from very small to larger, heavier objects. They vary in appearance, and include objects that are translucent and reflective. They include objects with highly non-convex shapes, soft and deformable parts, and parts that are inherently unsuitable for grasping (such as the bristles on a brush).
In analyzing the failure cases, we noticed the following patterns. In the test with replacement, many of the failed grasps were on the soft octopus toy (Fig.~\ref{fig:bin_unloading} (c)), where the robot would lift the octopus successfully by one of the tentacles, but it would slip out and fall back into the bin after lifting. Other failures were caused by the small round objects rolling into the corners of the bin, where they were difficult to reach. Since we impose hard bounds on the workspace to prevent the robot from colliding with the environment, in many of these cases it was actually impossible for the robot to grasp the object successfully, regardless of the policy.
In the bin emptying experiment, we found that many of the failures were due to the small black lock (Fig.~\ref{fig:bin_unloading} (a, right)) getting stuck in the corner of the bin, where it could not be grasped, resulting in multiple sequential failed attempts.


\paragraph{Clipped Double Q-Learning}
We find that using Clipped Double Q-Learning~\cite{td3} results in faster convergence in simulated experiments (Figure~\ref{fig:sim-dqn-graphs}) and is crucial for good performance in real experiments (Table~\ref{table:real-qlearn-ablation}). Experiments used the scripted termination. 
\begin{table}[h]
\begin{center}
\begin{tabular}{|p{13em}|p{5em}|}
\hline
Q-learning Method & Performance  \\
\hline
Double Q-learning & 63\% \\ %
\hline
Clipped Double Q-learning & 81\% \\ 
\hline
\end{tabular}
\end{center}
\caption{Off-policy performance with and without clipped Double-Q Learning.}
\label{table:real-qlearn-ablation}
\vspace{-0.25in}
\end{table}
\paragraph{Data efficiency}
As discussed in Section~\ref{sec:grasping_system} we collected 580k grasp attempts across 7 robots with a total of about 800 robot hours. Since we saved collected data on disk, we can study performance of a policy with less off-policy data. A dataset of 320k grasp attempts was generated by using data from the first 440 robot hours of data collection.
Table~\ref{tbl:real-data-efficiency} shows performance of off-policy training, using the best model configuration. With only 55\% of the original dataset, we reached 78\% grasp success, the same performance as our best supervised learning baseline, but using one third the number of grasps, and half the number of transitions. Further finetuning would likely yield a final policy that also reaches 96\% grasp success, with higher data efficiency but more on-robot finetuning time.
\begin{table}[h]
\begin{center}
\begin{tabular}{|p{7em}|p{5em}|}
\hline
Dataset Size & Performance  \\
\hline
580k grasps & 87\% \\ 
\hline
320k grasps & 78\% \\ 
\hline
\end{tabular}
\end{center}
\caption{Data efficiency.}
\label{tbl:real-data-efficiency}
\vspace{-0.25in}
\end{table}

==> arxiv_appendices/ablation_sim.tex <==
\begin{wrapfigure}{r}{0.22\textwidth}
\vspace{-0.4cm}
 \includegraphics[width=0.22\textwidth]{images/bullet}
\vspace{-0.4cm}
   \caption{Bullet Physics simulated environment.}
\vspace{-0.5cm}
\end{wrapfigure}
Robot experiments at large scale are excessively more time-consuming, complex, and uncertain than experimentation in a simulated environment.
We made extensive use of simulation for prototyping and ablation studies of our methods.

Our simulation environment is based on the Bullet Physics simulator~\citep{bullet} and mimics the setup shown in Fig.~\ref{fig:robot_setup_and_objects}. The simulated environment uses the configuration of the real Kuka IIWA arm, a similar looking bin, and a simulated over-the-shoulder camera. We used object models from the ShapeNet dataset ~\citep{shapenet}, scaled down to graspable sizes. Using our scalable distributed learning infrastructure (as discussed in Section~\ref{sec:qtopt}), we were able to generate data with up to 1,000 virtual robots running in parallel, and conduct a large scale experiment within a few hours. Both simulation and real used the same input modality, neural net architecture, and method of robotic control. Simulation was only used for prototyping, and all real world policies used only real data. We found that real world learning was generally much harder in terms of data requirements and time needed to train a good model, due to higher visual diversity, real world physics, and unmodeled properties of the real robot.

There are many parameters in our system which impact the final performance, data efficiency, generalization and emergence of rich behaviours. We split the factors into three large groups: QT-Opt specific parameters, grasping parameters, and data efficiency, which we discuss below.
\vspace{-0.1in}
\paragraph{QT-Opt specific parameters} include hyperparameters for Polyak averaging and the method of computing Bellman error. We found that $0.9999$ was the best Polyak averaging constant, and Double DQN performed better than Single DQN. Results are in Figure~\ref{fig:qtopt-comparison}. Note that although asymptotic performance is similar, the settings chosen seem to provide faster convergence and lower variance in grasp success. The latter is important for real experiments, where it is costly to evaluate the policy at multiple points. We also found that the cross-entropy loss performed better than the standard squared difference loss.

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots/polyak.pdf}
        \caption{All values of Polyak averaging provide stable training that reach similar performance, but higher values seem to converge faster and have smoother performance curves.}
        \label{fig:polyak-comparison}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/plots/dqn.pdf}
        \caption{Double DQN outperforms Single DQN on our task. Note that both are quite stable.}
        \label{fig:dqn-comparison}
    \end{subfigure}
    \caption{Comparison of Polyak averaging constants (a) and Single DQN vs Double DQN (b). Note these experiments do not include clipped Double Q-learning.}
    \label{fig:qtopt-comparison}
\end{figure}

\begin{figure}[h]
\centering
 \includegraphics[width=0.5\textwidth]{images/log-l2-loss}
   \caption{Loss function comparison in simulation}
\label{fig:sim-loss-graphs}
\end{figure}

Figure~\ref{fig:sim-dqn-graphs} compares Clipped Double DQN to standard Double DQN, showing Clipped Double DQN does slightly better. Note that although the difference in sim was small, we found performance was significantly better in the real world off-policy setting (see Table~\ref{table:real-qlearn-ablation}). The simulated setup uses 60 simulated, on-policy robots, which suggests the primary gains of Clipped Double DQN come when it is used with off-policy data.

\begin{figure}[h]
\centering
 \includegraphics[width=0.5\textwidth]{images/sim-td3-ablations}
   \caption{Comparison of DQN methods. See Appendix~\ref{sec:appendix_bellman_update} for clipped Double DQN definition.}
\label{fig:sim-dqn-graphs}
\vspace{-0.1in}
\end{figure}

\paragraph{Grasping parameters} describe the task specific MDP design, \ie state-action representations, closed-loop control and data generation policies. We found that differences in state representation as discussed in detail in Appendix~\ref{sec:appendix_state_action_reward}, greatly impacts performance. We compared models whose state is either a) just an image observation of the scene or b) a richer state comprising an image, the gripper aperture and distance between the gripper and the floor. Next, we studied discount factors and reward penalties. Finally, we compared a scripted episode stopping criterion to a learned termination action. In these experiments, we use 60 simulated robots, using \(\pi_{scripted}\) policy for the first 120K gradient update steps, then switching to the \(\pi_{noisy}\) policy with \(\epsilon=0.2\). These exploration policies are explained in Appendix~\ref{sec:appendix_exploration}. The grasp performance is evaluated continuously and concurrently as training proceeds by running the \(\pi_{eval}\) policy on 100 separate simulated robots and aggregating 700 grasps per policy for each model checkpoint.

\begin{table}[h]
\begin{center}
\begin{tabular}{ |p{7em}|p{5em}|p{5em}|p{5em}|p{5em}|p{5em}| } 
\hline
State & Termination action & Intermediate reward & Discount factor & Perf. at 300K steps & Perf. at 1M steps\\
\hline
\multirow{3}{7em}{Image+gripper status+height}
& No & -0.05 & 0.9 & 75\%& 95\% \\ %
& No & 0 & 0.9 & 68\%& 92\% \\ %
& No & 0 & 0.7 & 50\%& 90\% \\ %
\hline
Image only & No & -0.05 & 0.9 & 25\%& 81\% \\ %
\hline
Image+gripper status+height & Yes & -0.05 & 0.9 & 67\%& 94\% \\
\hline
\end{tabular}
\end{center}
\caption{Simulation studies for tuning grasping task parameters}
\label{table:sim-grasping-ablation}
\end{table}

\begin{figure}[h]
\centering
 \includegraphics[width=0.5\textwidth]{images/sim_grasping_ablations_graph}
   \caption{Performance graphs of simulation studies for tuning grasping task parameters}
\label{fig:sim-graphs}
\vspace{-0.05in}
\end{figure}
The results in Table~\ref{table:sim-grasping-ablation} show that richer state representation results in faster convergence and better final performance. A small reward penalty does much better than decreasing the discount factor. Finally, giving the policy greater control over the episode termination yields performance on par with the engineered termination condition.

We put special focus on the termination action: by letting the policy decide when to terminate, the policy has more potential to keep trying a grasp until it is confident the grasp is stable. We argue that explicitly learning a termination action would be beneficial for many manipulation tasks, since it makes the design of the MDP easier and it forces the policy to truly understand the goal of the task.


\paragraph{Data efficiency} 
Interestingly, our algorithm is more data efficient than the supervised learning based algorithm from ~\citet{levine16} work, achieving higher grasp success with fewer robots continuously generating training data (see Table~\ref{table:sim-data-eff}).

\begin{table}[h]
\begin{center}
\begin{tabular}{ |p{7em}|p{5em}|p{3em}| } 
\hline
Name & Sim Robots &
Success \\
\hline
\multirow{2}{7em}{QT-Opt (ours)} & 30 & 88\% \\
&60 & 95\% \\
\hline
\multirow{3}{7em}{\citet{levine16}} & 60 & 55\% \\
& 280 & 71\% \\
& 1000 & 85\% \\
 \hline
\end{tabular}
\end{center}
\caption{Data efficiency comparison in simulation.}
\label{table:sim-data-eff}
\vspace{-0.25in}
\end{table}
We argue that the algorithm from ~\citet{levine16} is less data efficient because it optimizes a proxy objective of 1-step classification accuracy, which values all data points equally. Our QT-Opt policy values data points based on how they influence reward. This focuses optimization on pivotal decision points that are very important to get right, such as learning when to close the gripper. Doing so lets the model optimize grasp success more efficiently.

\subsection{Effect of Off-Policy Training on Performance}
\label{sec:appendix_off_policy}
\input{arxiv_appendices/appendix_off_policy}

